Go with the Flow: Adaptive Control for Neural ODEs

Despite their elegant formulation and lightweight memory cost, neural ordinary differential equations (NODEs) suffer from known representational limitations. In particular, the single flow learned by NODEs cannot express all homeomorphisms from a given data space to itself, and their static weight parameterization restricts the type of functions they can learn compared to discrete architectures with layer-dependent weights. Here, we describe a new module called neurally controlled ODE (N-CODE) designed to improve the expressivity of NODEs. The parameters of N-CODE modules are dynamic variables governed by a trainable map from initial or current activation state, resulting in forms of open-loop and closed-loop control, respectively. A single module is sufficient for learning a distribution on non-autonomous flows that adaptively drive neural representations. We provide theoretical and empirical evidence that N-CODE circumvents limitations of previous NODEs models and show how increased model expressivity manifests in several supervised and unsupervised learning problems. These favorable empirical results indicate the potential of using data- and activity-dependent plasticity in neural networks across numerous domains.

==> drafts.tex <==
 ###### abstract ########
 
 %Despite their elegant formulation and lightweight memory cost, neural ordinary differential equations (neural ODEs), suffer from well-known representational limitations. In particular, the single neural flow learned by NODEs cannot approximate all homeomorphisms from a given data space to itself. Here, we attempt to alleviate this limitation by proposing a new continuous-time representation learning framework called neurally-controlled ODE (N-CODE). In our framework, a different, generally non-autonomous neural flow is output \emph{per datum} so that the model dynamics represent an input-dependent control system. We describe both closed-loop and open-loop versions of this framework, in which flows depend on the system state or not, respectively. We provide empirical and theoretical evidence that these data-dependent neural flows greatly increase the expressivity of our system vs other continuous-time methods and show how this increased expressivity manifests as improved peformance in several domains. In supervised learning, we demonstrate that our framework achieves better performance than neural ODEs as measured by both training speed and testing accuracy. In unsupervised learning, we show how data-dependent flows can act as powerful latent representations which greatly decrease the error of a vanilla image autoencoder, leading to state-of-the art image reconstruction on CIFAR-10.
\newline

%Despite their elegant formalism and lightweight memory cost, neural ordinary differential equations (neural ODEs), suffer from known representational limitations. In particular, the single flow learned by original NODEs cannot express all homeomorphisms from a given data space to itself and their static weight parameterization restricts the types of layered, feedforward architectures they can approximate. Here, we attempt to alleviate these representational limitations by proposing neurally-controlled ODE (N-CODE) modules. In this framework, we consider neural ODE parameters as dynamic variables driven by a control system that depends on input data or activation state, resulting in forms of \textit{open-loop} and \textit{closed-loop} control respectively. This framework enable to learn, with the same module, a push-forward distribution of feature transformative flows. We provide empirical and theoretical evidence that such adaptive neural flows circumvent limitations of previous models and show how increased model expressivity manifests in several domains. In supervised learning, we demonstrate that our framework achieves better performance than neural ODEs as measured by both training speed and testing accuracy. In unsupervised learning, we apply this control perspective to an image autoencoder endowed with a latent transformation flow, greatly improving the representational power over a vanilla model and leading to state-of-the art image reconstruction on CIFAR-10.
\newline

%Despite their elegant formulation and lightweight memory cost, neural ordinary differential equations (NODEs) suffer from known representational limitations. In particular, the single flow learned by NODEs cannot express all homeomorphisms from a given data space to itself and their static weight parameterization restricts the types of layered, feedforward architectures they can approximate. Here, we describe a new approach called neurally-controlled ODEs (N-CODE) designed to alleviate these expressivity limitations. N-CODE modules parameters are dynamic variables governed by a trainable control system that maps initial (open-loop) or current (closed-loop) activation state to a distribution of non-autonomous flows that optimally drives neural representations. We provide theoretical and empirical evidence that N-CODE modules circumvent limitations of previous models and show how increased model expressivity manifests in several domains. In supervised learning, we demonstrate that our framework achieves better performance than NODEs as measured by both training speed and testing accuracy. In unsupervised learning, we apply this control perspective to an image autoencoder endowed with a latent transformation flow, greatly improving the representational power over a vanilla model and leading to state-of-the art image reconstruction on CIFAR-10.




%Neural Ordinary Differential Equations (ODEs) proposed artificial neural modules as differentiable functions describing continuous flows over the feature/activation space. Despite their elegant formulation and lightweight training cost due to the adjoint method, their current formulation leads to learning a single time-constant flow which cannot not be universal approximator for homeomorphic functions. Here, we present a new framework for Neural ODE, called N-CODE, where we consider Neural ODE module parameters as dynamic variables dependant on data/activity state instead of a fixed set of weights. We augment a NODE module parameters with control mechanisms given data or activation state recovering forms of \texit{open-loop} and \texit{closed-loop} control respectively, yielding more flexible feature transformation flows. We show that this augmentation breaks the universal approximation limitation of non-autonomous Neural ODE, i.e where the dynamics depends explicitly on time. In supervised learning, we demonstrate that this mechanism improve Neural ODE performance in both training speed and accuracy. In unsupervised learning, this control perspective inspired a latent transformation layer that greatly improves the representational power of a vanilla image autoencoder, leading to state-of-the art image reconstruction on CIFAR-10.
 
 ########################
